Root Cause Analysis for Microservice System based on Causal Inference: How Far Are We?

Microservice architecture has become a popular architecture adopted by many cloud applications. However, identifying the root cause of a failure in microservice systems is still a challenging and time-consuming task. In recent years, researchers have introduced various causal inference-based root cause analysis methods to assist engineers in identifying the root causes. To gain a better understanding of the current status of causal inference-based root cause analysis techniques for microservice systems, we conduct a comprehensive evaluation of nine causal discovery methods and twenty-one root cause analysis methods. Our evaluation aims to understand both the effectiveness and efficiency of causal inference-based root cause analysis methods, as well as other factors that affect their performance. Our experimental results and analyses indicate that no method stands out in all situations; each method tends to either fall short in effectiveness, efficiency, or shows sensitivity to specific parameters. Notably, the performance of root cause analysis methods on synthetic datasets may not accurately reflect their performance in real systems. Indeed, there is still a large room for further improvement. Furthermore, we also suggest possible future work based on our findings.

==> experiments.tex <==
\subsection{Data}

\subsubsection{Synthetic and semi-synthetic data}

Three datasets from three research works are used: CIRCA, RCD, and CausIL, in table \ref{tab:synthetic-data}.

\begin{table}[H]
\centering
\caption{Synthetic data information}
\label{tab:synthetic-data}
\begin{tabular}{|l|l|r|l|l|l|}
\hline
\textbf{Name} &
  \textbf{Graph Size} &
  \multicolumn{1}{l|}{\textbf{Length}} &
  \textbf{\begin{tabular}[c]{@{}l@{}}Simulating\\ real system?\end{tabular}} &
  \textbf{Fault?} &
  \textbf{Data type} \\ \hline
CIRCA &
  \begin{tabular}[c]{@{}l@{}}- 5 nodes x 10 edges\\ - 10 nodes x 20 edges\\ - 50 nodes x 100 edges\\ - 100 nodes x 500 edges\end{tabular} &
  4000 &
  N &
  Y &
  float \\ \hline
RCD    & \begin{tabular}[c]{@{}l@{}}- 5 nodes\\ - 10 nodes\\ - 50 nodes\\ - 100 nodes\end{tabular} & 4000 & N & Y & int   \\ \hline
CausIL & \begin{tabular}[c]{@{}l@{}}- 10 nodes\\ - 50 nodes\end{tabular}                           & 4000 & Y & N & float \\ \hline
\end{tabular}
\end{table}



\subsubsection{Collected Data from benchmark systems}

Three popular benchmark systems are deployed, injected faults and collected data, table \ref{tab:real-data}.


\begin{table}[H]
\centering
\caption{Collected data from benchmark systems}
\label{tab:real-data}
\begin{tabular}{|l|r|r|r|r|r|r|}
\hline
\textbf{System name} &
  \multicolumn{1}{l|}{\textbf{No. services}} &
  \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}No. injected\\ services\end{tabular}}} &
  \multicolumn{1}{l|}{\textbf{No. fault}} &
  \textbf{Duration} &
  \multicolumn{1}{l|}{\textbf{No. cases}} &
  \textbf{No. metrics} \\ \hline
Sock-shop       & 11 & 5 & 4 & 1 hour & 58 & 399               \\ \hline
Online-boutique & 12 & 5 & 2 & 1 hour & 50 & 49 \\ \hline
Train-ticket    & 64 & 2 & 4 & 1 hour & 31 & 1049             \\ \hline
\end{tabular}
\end{table}

\subsection{Evaluation Metrics}

For the graph construction, we assess the causal graph using the following measures, as described in previous studies.
\begin{itemize}
    \item Precision, Recall, and F1-score on the skeleton of the graph. This metric aims to evaluate the accuracy of the edges in the graph without considering their directions.
    \item Precision, Recall, and F1-score on the full graph. This metric takes into account the causal orientations of the edges and penalizes for incorrectly estimated directions of correctly identified adjacencies.
    \item The Structural Hamming Distance (SHD) indicates the number of changes needed to transform the estimated causal graph into the true graph.
\end{itemize}


For the root cause analysis task, we evaluate the performance of a method through the recall with the top-k results, denoted as $Acc@K$, following existing works.

We also record the processing time of the algorithms.

